Estimation of instrument and noise parameters for inverse problem based on prior diffusion model

This article addresses the issue of estimating observation parameters (response and error parameters) in inverse problems. The focus is on cases where regularization is introduced in a Bayesian framework and the prior is modeled by a diffusion process. In this context, the issue of posterior sampling is known to be thorny, and a recent paper proposes a notably simple and effective solution. Additionally, it opens an remarkable flexibility when it comes to estimating observation parameters. The proposed strategy enables to define an optimal estimator for both observation parameters and image of interest. Furthermore, the strategy provides a means for uncertainty quantification. In addition, MCMC algorithms allow for the computation of estimates and properties of posteriors, while offering some guarantees. The paper presents several numerical experiments that clearly confirm the computational efficiency and the quality of both estimates and uncertainty quantification.

==> Macros/abrege.tex <==
% TEX 7(ascii) bits
%
% ABREGE.tex
% LaTeX document
% Author: J.I. 
% Date  : Juillet 1996
%
% Raccourcis d'expressions très usitées
%
% Derniere modif le 10-07-96
%
%
% ==> OK, JFG -- 26/04/2010
%

% Raccourci pour \XS
\def\XS{\xspace}

%%%%%%%%%%%%%%%%%%% Pour definir nouvelle commande de changement de taille
\RequirePackage{ifthen}
\RequirePackage{calc}

\newcommand{\taille}[1][\scad]{%
\ifthenelse{#1 = -5}{}{}%
\ifthenelse{#1 = -4}{\tiny}{}%
\ifthenelse{#1 = -3}{\scriptsize}{}%
\ifthenelse{#1 = -2}{\footnotesize}{}%
\ifthenelse{#1 = -1}{\small}{}%
\ifthenelse{#1 = 0}{\normalsize}{}%
\ifthenelse{#1 = 1}{\large}{}%
\ifthenelse{#1 = 2}{\Large}{}%
\ifthenelse{#1 = 3}{\LARGE}{}%
\ifthenelse{#1 = 4}{\huge}{}%
\ifthenelse{#1 = 5}{\Huge}{}}

\newboolean{@serif}
\setboolean{@serif}{true}
\def\scad{-5} % scadefaultsize

\newcounter{taille}
\newcommand{\sca}[2][\scad]{\setcounter{taille}{#1}%
  \ifthenelse{\boolean{@serif}}
  {{\taille[\thetaille]\textsc{#2}}}
  {\setcounter{taille}{\value{taille}-1}{\uppercase{\taille[\thetaille]#2}}}}


%%% RACCOURCIS DIVERS %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

% Mise en commentaire rapide !
	\def\Rem#1{}                    % rem{bla bla bla}

% References automatiquement entre parenthese
	%\def\reff#1{\XS(\ref{#1})}
	%\def\refs#1{section~\ref{#1}}
	%\def\refS#1{Section~\ref{#1}}

% Nettoyage
	%\newcommand{\clearemptydoublepage}{\newpage{\pagestyle{empty}\cleardoublepage}}  

% Numéro (pour biblio)
	%\def\numero{n°}
	\def\numero{n\textsuperscript{o}\,}
	%\def\Numero{N°}
	\def\numero{N\textsuperscript{o}\,}

% Majuscules
	\def\UP#1{\uppercase{#1}}       % majuscules
	\def\up#1{\uppercase{#1}}       % majuscules

% References automatiquement entre parenthese
 \def\reff#1{\XS(\ref{#1})}
 %\def\refs#1{section~\ref{#1}}
 %\def\refS#1{Section~\ref{#1}}

%%% RACCOURCIS d'italique, locutions,... %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\def\adhoc{\textit{ad hoc}\XS}
\def\apost{\textit{a posteriori}\XS}
\def\Apost{\textit{A posteriori}\XS}
\def\APost{\textit{A Posteriori}\XS}
\def\post{\textit{posterior}\XS}
\def\Post{\textit{Posterior}\XS}
\def\afortio{\textit{a fortiori}\XS}
\def\Afortio{\textit{A fortiori}\XS}
\def\aprio{\textit{a priori}\XS}
\def\Aprio{\textit{A priori}\XS}
\def\Cad{C'est-\`a-dire\XS}
\def\cad{c'est-\`a-dire\XS}
\def\Cpq{C'est pourquoi\XS}
\def\cpq{c'est pourquoi\XS}
\def\coeur{c{\oe}ur\XS}
\def\cf{\textit{cf.}\XS}
\def\eg{\textit{e.g.,}\XS}
\def\etal{\textit{et al.}\XS}
\def\etc{\textit{etc}\XS} %\def\etc{\textit{etc\dots}\XS}
\def\etcoll{{\textit et coll.}\XS}
\def\idem{\textit{idem}\XS}
\def\ie{\textit{i.e.,}\XS}
\def\iid{i.i.d.\XS}
\def\infine{\textit{in fine}\XS}
\def\insit{\textit{in situ}\XS}
\def\inviv{\textit{in vivo}\XS}
\def\oeuvre{{\oe}uvre\XS}
\def\oeuvres{{\oe}uvres\XS}
\def\oeil{{\oe}il\XS}
\def\recto{\textit{recto}\XS}
\def\Toeplitz{T{\oe}plitz\XS}
\def\vav{vis-\`a-vis\XS}
\def\via{\textit{via}\XS}
\def\vic{\textit{vice-versa}\XS}
\def\verso{\textit{verso}\XS}
\def\vs{\textit{vs}\XS}
\def\versus{\textit{versus}\XS}
\def\ssi{\textit{si et seulement si}\XS}
\def\strsen{\textit{stricto sensu}\XS}
\def\wrt{w.r.t.\XS}

\def\ier{$^{\text{\small er}}$\XS}
\def\iere{$^{\text{\small re}}$\XS}
\def\ieme{$^{\text{\small e}}$\XS}

\def\primo{\ensuremath{1^{\oD}}\XS}
\def\secundo{\ensuremath{2^{\oD}}\XS}
\def\tertio{\ensuremath{3^{\oD}}\XS}
\def\quatro{\ensuremath{4^{\oD}}\XS}

	\def\MALDI{Matrix-Assisted Laser Desorption/Ionisation\XS}
	\newcommand{\maldi}[1][\scad]{\sca[#1]{maldi}\XS}

	\def\BHIPRO{Bayesian Hierarchical Inversion in Proteomics\XS}
	\newcommand{\bhipro}[1][\scad]{\sca[#1]{bhi-pro}\XS}

	\def\BNPSI{Bayesian Non-Parametreic in Signal-Image\XS}
	\newcommand{\bnpsi}[1][\scad]{\sca[#1]{bnp-si}\XS}

%%% ACRONYMES %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

% Divers 
	\newcommand{\art}[1][\scad]{\sca[#1]{art}\XS}
	\newcommand{\cnd}[1][\scad]{\sca[#1]{cnd}\XS}
	\newcommand{\ndt}[1][\scad]{\sca[#1]{ndt}\XS}
	\newcommand{\gnc}[1][\scad]{\sca[#1]{gnc}\XS}
	\newcommand{\mfa}[1][\scad]{\sca[#1]{mfa}\XS}
	\newcommand{\map}[1][\scad]{\sca[#1]{map}\XS}

	\newcommand{\icm}[1][\scad]{\sca[#1]{icm}\XS}
	\newcommand{\icd}[1][\scad]{\sca[#1]{icd}\XS}
	\newcommand{\rsb}[1][\scad]{\sca[#1]{rsb}\XS}
	\newcommand{\snr}[1][\scad]{\sca[#1]{snr}\XS}
	\newcommand{\fft}[1][\scad]{\sca[#1]{fft}\XS}
	\newcommand{\fftdd}[1][\scad]{\sca[#1]{fft-2d}\XS}
	\newcommand{\ifft}[1][\scad]{\sca[#1]{ifft}\XS}
	\newcommand{\dsp}[1][\scad]{\sca[#1]{dsp}\XS}

	\newcommand{\dess}[1][\scad]{\sca[#1]{dess}\XS}
	\newcommand{\dea}[1][\scad]{\sca[#1]{dea}\XS}
	\newcommand{\deug}[1][\scad]{\sca[#1]{deug}\XS}
	\newcommand{\deust}[1][\scad]{\sca[#1]{deust}\XS}
	\newcommand{\iut}[1][\scad]{\sca[#1]{iut}\XS}
	\newcommand{\iup}[1][\scad]{\sca[#1]{iup}\XS}
	\newcommand{\ects}[1][\scad]{\sca[#1]{ects}\XS}

	\newcommand{\ufr}[1][\scad]{\sca[#1]{ufr}\XS}
	\newcommand{\uf}[1][\scad]{\sca[#1]{uf}\XS}
	\newcommand{\upr}[1][\scad]{\sca[#1]{upr}\XS}

	\newcommand{\gbm}[1][\scad]{\sca[#1]{gbm}\XS}
	\newcommand{\irmf}[1][\scad]{\sca[#1]{irm-f}\XS}
	\newcommand{\irm}[1][\scad]{\sca[#1]{irm}\XS}
	\newcommand{\rmn}[1][\scad]{\sca[#1]{rmn}\XS}
	\newcommand{\eeg}[1][\scad]{\sca[#1]{eeg}\XS}
	\newcommand{\meg}[1][\scad]{\sca[#1]{meg}\XS}


% Transformées
	\newcommand{\tf}[1][\scad]{\sca[#1]{tf}\XS}
	%\newcommand{\sf}[1][\scad]{\sca[#1]{sf}\XS}
	\def\sf{\textsc{sf}\XS}
	\newcommand{\tl}[1][\scad]{\sca[#1]{tl}\XS}
	\newcommand{\tz}[1][\scad]{\sca[#1]{tz}\XS}
	\newcommand{\tpsc}[1][\scad]{\sca[#1]{tc}\XS}
	\newcommand{\tpsd}[1][\scad]{\sca[#1]{td}\XS}

% Operating Systemes 
	\newcommand{\linux}[1][\scad]{\sca[#1]{Linux}\XS}
	\newcommand{\unix}[1][\scad]{\sca[#1]{Unix}\XS}
	\newcommand{\msdos}[1][\scad]{\sca[#1]{msdos}\XS}
	\newcommand{\sunos}[1][\scad]{\sca[#1]{Sunos}\XS}
	\newcommand{\hupux}[1][\scad]{\sca[#1]{hp-ux}\XS}
	\newcommand{\vms}[1][\scad]{\sca[#1]{vms}\XS}
	\newcommand{\solaris}[1][\scad]{\sca[#1]{Solaris}\XS}
	\newcommand{\winnt}[1][\scad]{\sca[#1]{Windows-nt}\XS}
	\newcommand{\vmware}[1][\scad]{\sca[#1]{vmware}\XS}
	\newcommand{\win}[1][\scad]{\sca[#1]{Windows}\XS}

% Calcul scientifique
	\newcommand{\labview}[1][\scad]{\sca[#1]{Labview}\XS}
	\newcommand{\matlab}[1][\scad]{\sca[#1]{Matlab}\XS}
	\newcommand{\maple}[1][\scad]{\sca[#1]{Maple}\XS}
	\newcommand{\mathe}[1][\scad]{\sca[#1]{Mathematica}\XS}
	\newcommand{\idl}[1][\scad]{\sca[#1]{Idl}\XS}

% Langages
	\newcommand{\cmex}[1][\scad]{\sca[#1]{Cmex}\XS}
	\newcommand{\pascal}[1][\scad]{\sca[#1]{Pascal}\XS}
	\newcommand{\java}[1][\scad]{\sca[#1]{Java}\XS}
	\newcommand{\lisp}[1][\scad]{\sca[#1]{Lisp}\XS}
	\newcommand{\forts}[1][\scad]{\sca[#1]{Fortran}{\footnotesize 77}\XS}
	\newcommand{\fortq}[1][\scad]{\sca[#1]{Fortran}{\footnotesize 90}\XS}
	\newcommand{\ada}[1][\scad]{\sca[#1]{Ada}\XS}
	\newcommand{\eiffel}[1][\scad]{\sca[#1]{Eiffel}\XS}
	\newcommand{\tcsh}[1][\scad]{\sca[#1]{tcsh}\XS}
	\newcommand{\bash}[1][\scad]{\sca[#1]{bash}\XS}
	\newcommand{\lgc}[1][\scad]{\sca[#1]{C}\XS}
	\newcommand{\cpp}[1][\scad]{\sca[#1]{C}{\footnotesize ++}\XS}

% Congres
	\newcommand{\gretsi}[1][\scad]{\sca[#1]{gretsi}\XS}
	\newcommand{\maxent}[1][\scad]{\sca[#1]{maxent}\XS}
	\newcommand{\icip}[1][\scad]{\sca[#1]{icip}\XS}
	\newcommand{\icassp}[1][\scad]{\sca[#1]{icassp}\XS}
	\newcommand{\spie}[1][\scad]{\sca[#1]{spie}\XS}
	%\newcommand{\gdr}[1][\scad]{\sca[#1]{gdr--prc~isis}\XS}
	\newcommand{\gdr}[1][\scad]{\sca[#1]{gdr~isis}\XS}
	\newcommand{\rfia}[1][\scad]{\sca[#1]{rfia}\XS}
	\newcommand{\eusipco}[1][\scad]{\sca[#1]{eusipco}\XS}

% Restes
	\newcommand{\leti}[1][\scad]{\sca[#1]{leti}\XS}
	\newcommand{\cesta}[1][\scad]{\sca[#1]{cesta}\XS}
	\newcommand{\minatec}[1][\scad]{\sca[#1]{minatec}\XS}
	\newcommand{\stic}[1][\scad]{\sca[#1]{stic}\XS}
	\newcommand{\pc}[1][\scad]{\sca[#1]{pc}\XS}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% Ajout de famouss.tex
% modif le 25/5/2000 Phiphi
% GPInuts - Famous people - VIP
%
\newcommand{\beaunom}[4][0]{{\taille[#1]#2 \uppercase{#3}}{\sca[#1]{#4}}\XS}

%\newcommand{\MA}[1][\scad]{{\taille[#1]Marc \uppercase{A}}% 
%{\sca[#1]{llain}\XS}}
\newcommand{\AuGi}[1][\scad]{\beaunom[#1]{Audrey}{G}{iremus}}

\newcommand{\AB}[1][\scad]{\beaunom[#1]{Amandine}{B}{lanc}}
\newcommand{\ABF}[1][\scad]{\beaunom[#1]{Amandine}{B}{lanc~--~Fusco}}
\newcommand{\AAB}[1][\scad]{\beaunom[#1]{Alain}{A}{bergel}}
\newcommand{\AnBa}[1][\scad]{\beaunom[#1]{Andrei}{B}{arbos}}
\newcommand{\AC}[1][\scad]{\beaunom[#1]{Alain}{C}{oulais}}
\newcommand{\AH}[1][\scad]{\beaunom[#1]{Alain}{H}{erment}}
\newcommand{\AG}[1][\scad]{\beaunom[#1]{Audrey}{G}{iremus}}
\newcommand{\AHz}[1][\scad]{\beaunom[#1]{Aur\'elien}{H}{azart}}
\newcommand{\AMD}[1][\scad]{\beaunom[#1]{Ali}{M}{ohammad--Djafari}}
\newcommand{\AR}[1][\scad]{\beaunom[#1]{Andrea}{R}{idolfi}}
\newcommand{\BDuc}[1][\scad]{\beaunom[#1]{Bernard}{D}{uch\^ene}}
\newcommand{\BH}[1][\scad]{\beaunom[#1]{Benjamin}{H}{arrou\'e}}
\newcommand{\CH}[1][\scad]{\beaunom[#1]{Christian}{H}{einrich}}
\newcommand{\CS}[1][\scad]{\beaunom[#1]{Charles}{S}{oussen}}
\newcommand{\CV}[1][\scad]{\beaunom[#1]{Cornelia}{V}{acar}}
\newcommand{\DLB}[1][\scad]{\beaunom[#1]{Denis}{L}{e Bihan}}
\newcommand{\FA}[1][\scad]{\beaunom[#1]{Fr\'ed\'eric}{A}{uch\`ere}}
\newcommand{\FC}[1][\scad]{\beaunom[#1]{Fr\'ed\'eric}{C}{hampagnat}}
\newcommand{\FrCa}[1][\scad]{\beaunom[#1]{Fran\c{c}ois}{C}{aron}}
\newcommand{\FL}[1][\scad]{\beaunom[#1]{Franck}{L}{etimonier}}
\newcommand{\FV}[1][\scad]{\beaunom[#1]{Francisco}{V}{arela}}
\newcommand{\FDU}[1][\scad]{\beaunom[#1]{Fr\'ed\'eric}{D}{ublanchet}}
\newcommand{\FB}[1][\scad]{\beaunom[#1]{Fran\c{c}ois}{B}{oulanger}}
\newcommand{\FO}[1][\scad]{\beaunom[#1]{Fran\c{c}ois}{O}{rieux}}
\newcommand{\GDE}[1][\scad]{\beaunom[#1]{Guy}{D}{emoment}}
\newcommand{\GS}[1][\scad]{\beaunom[#1]{Gr\'egory}{S}{trubel}}
\newcommand{\GB}[1][\scad]{\beaunom[#1]{Guillaume}{B}{ourmaud}}
\newcommand{\GLB}[1][\scad]{\beaunom[#1]{Guy}{L}{e Besnerais}}
\newcommand{\GL}[1][\scad]{\beaunom[#1]{Guilaine }{L}{agache}}
\newcommand{\GR}[1][\scad]{\beaunom[#1]{Gilles}{R}{ochefort}}
\newcommand{\HC}[1][\scad]{\beaunom[#1]{Herv\'e}{C}{arfantan}}
\newcommand{\HS}[1][\scad]{\beaunom[#1]{Hichem}{S}{noussi}}
\newcommand{\JB}[1][\scad]{\beaunom[#1]{Julien}{B}{oissy}}
\newcommand{\JCV}[1][\scad]{\beaunom[#1]{Jean--Claude}{V}{ial}}
\newcommand{\JFB}[1][\scad]{\beaunom[#1]{Jean--Fran\c{c}ois}{B}{ercher}}
\newcommand{\JFG}[1][\scad]{\beaunom[#1]{Jean\,--\,Fran\c{c}ois}{G}{iovan\-nel\-li}}
\newcommand{\JFM}[1][\scad]{\beaunom[#1]{Jean--Fran\c{c}ois}{M}{angin}}
\newcommand{\JI}[1][\scad]{\beaunom[#1]{J\'er\^ome}{I}{dier}}
\newcommand{\JML}[1][\scad]{\beaunom[#1]{Jean\,--\,Marie}{L}{alande}}
\newcommand{\JeSo}[1][\scad]{\beaunom[#1]{Jessica}{S}{odjo}}
\newcommand{\JBP}[1][\scad]{\beaunom[#1]{Jean-Baptiste}{P}{oline}}
\newcommand{\KS}[1][\scad]{\beaunom[#1]{Ken}{S}{auer}}
\newcommand{\LG}[1][\scad]{\beaunom[#1]{Line}{G}{arnero}}
\newcommand{\MA}[1][\scad]{\beaunom[#1]{Marc}{A}{llain}}
\newcommand{\MF}[1][\scad]{\beaunom[#1]{Marc}{F}{ayolle}}
\newcommand{\Mimi}[1][\scad]{\beaunom[#1]{Myriam}{F}{iani}}
\newcommand{\MN}[1][\scad]{\beaunom[#1]{Mila}{N}{ikolova}}
\newcommand{\MP}[1][\scad]{\beaunom[#1]{Marcelo}{P}{ereyra}}
\newcommand{\NBA}[1][\scad]{\beaunom[#1]{Nicolas}{B}{arbey}}
\newcommand{\OF}[1][\scad]{\beaunom[#1]{Olivier}{F}{\'eron}}
\newcommand{\PC}[1][\scad]{\beaunom[#1]{Philippe}{C}{iuciu}}
\newcommand{\PG}[1][\scad]{\beaunom[#1]{Pierre}{G}{rangeat}}
\newcommand{\PS}[1][\scad]{\beaunom[#1]{Pascal}{S}{zacherski}}
\newcommand{\PM}[1][\scad]{\beaunom[#1]{Pierre}{M}{invielle}}
\newcommand{\RB}[1][\scad]{\beaunom[#1]{Redha}{B}{oubertakh}}
\newcommand{\SB}[1][\scad]{\beaunom[#1]{St\'ephane}{B}{rette}}
\newcommand{\SG}[1][\scad]{\beaunom[#1]{St\'ephane}{G}{autier}}
\newcommand{\SBA}[1][\scad]{\beaunom[#1]{Sylvain}{B}{ailet}}
\newcommand{\TM}[1][\scad]{\beaunom[#1]{Thierry}{M}{artin}}
\newcommand{\TR}[1][\scad]{\beaunom[#1]{Thomas}{R}{odet}}
\newcommand{\TB}[1][\scad]{\beaunom[#1]{Thomas}{B}{enoudiba}}
\newcommand{\VS}[1][\scad]{\beaunom[#1]{Vincent}{S}{amson}}
\newcommand{\YA}[1][\scad]{\beaunom[#1]{Yoann}{A}{ltman}}
\newcommand{\YB}[1][\scad]{\beaunom[#1]{Yannick}{B}{erthoumieu}}
\newcommand{\YG}[1][\scad]{\beaunom[#1]{Yves}{G}{oussard}}



% Acronymes et raccourcis

	\def\EEA{\'Electronique \`Electrotechnique Automatique\XS}
	\newcommand{\eea}[1][\scad]{\sca[#1]{eea}\XS}

	\def\IMA{Institut de Maintenance A\'eronautique\XS}
	\newcommand{\ima}[1][\scad]{\sca[#1]{ima}\XS}

	\def\EAPSI{\'Electronique, Automatique, Productique et Signal-Image\XS}
	\newcommand{\eapsi}[1][\scad]{\sca[#1]{eapsi}\XS}

	\def\GSAT{G\'enie des Syst\`emes pour l'A\'eronautique et les Transports\XS}
	\newcommand{\gsat}[1][\scad]{\sca[#1]{gsat}\XS}

	\def\ANR{Agence Nationale de la Recherche\XS}
	\newcommand{\anr}[1][\scad]{\sca[#1]{anr}\XS}

	\def\ENSEIRB{\'Ecole Nationale Sup\'erieure d'\'Electronique, Informatique et T\'el\'ecommunications de Bordeaux\XS}
	\newcommand{\enseirb}[1][\scad]{\sca[#1]{enseirb}\XS}
	%
	\newcommand{\matmeca}[1][\scad]{\sca[#1]{matmeca}\XS}

	\def\ENSC{\'Ecole Nationale Sup\'erieure de Cognitique\XS}
	\newcommand{\ensc}[1][\scad]{\sca[#1]{ensc}\XS}

	\def\ATS{Automatique et Traitement du Signal\XS}
	\newcommand{\ats}[1][\scad]{\sca[#1]{ats}\XS}

	\def\THCS{Traitement Harmonique et Contr\^ole du Signal\XS}
	\newcommand{\thcs}[1][\scad]{\sca[#1]{thcs}\XS}

	\def\TE{travaux d'\'etudes\XS}
	\newcommand{\te}[1][\scad]{\sca[#1]{te}\XS}

	\def\TD{travaux dirig\'es\XS}
	\def\GTD{Travaux dirig\'es\XS}
	\newcommand{\td}[1][\scad]{\sca[#1]{td}\XS}

	\def\TP{travaux pratiques\XS}
	\def\GTP{Travaux pratiques\XS}
	\newcommand{\tp}[1][\scad]{\sca[#1]{tp}\XS}

	\def\TDAO{travaux dirig\'es assist\'es sur ordinateur\XS}
	\newcommand{\tdao}[1][\scad]{\sca[#1]{tdao}\XS}

	\def\ATER{Attach\'e temporaire d'enseignement et de recherche}
	\newcommand{\ater}[1][\scad]{\sca[#1]{ater}\xspace}

	\def\ADDOC{Agir pour les Doctorants et les jeunes Docteurs\XS}
	\newcommand{\addoc}[1][\scad]{\sca[#1]{addoc}\XS}

	\def\SHFJ{Service Hospitalier Fr\'ed\'eric Joliot\XS}
	\newcommand{\shfj}[1][\scad]{\sca[#1]{shfj}\XS}

	\def\UNAF{Unit\'e de Neuroimagerie Anatomo Fonctionnelle\XS}
	\newcommand{\unaf}[1][\scad]{\sca[#1]{unaf}\XS}

	\def\CHU{Centre Hospitalier Universitaire\XS}
	\newcommand{\chu}[1][\scad]{\sca[#1]{chu}\XS}

	\def\LIF{Laboratoire d'Imagerie Fonctionnelle\XS}
	\newcommand{\lif}[1][\scad]{\sca[#1]{lif}\XS}

	\def\CEA{Commissariat \`a l'\'Enegie Atomique\XS}
	\newcommand{\cea}[1][\scad]{\sca[#1]{cea}\XS}

	\def\DRM{D\'epartement de Recherche M\'edicale\XS}
	\newcommand{\drm}[1][\scad]{\sca[#1]{drm}\XS}

	\def\DAM{Direction des Affaires Militaires\XS}
	\newcommand{\dam}[1][\scad]{\sca[#1]{dam}\XS}

	\def\DSV{Direction des Sciences du Vivant\XS}
	\newcommand{\dsv}[1][\scad]{\sca[#1]{dsv}\XS}

	\def\CNRS{Centre National de la Recherche Scientifique\XS}
	\newcommand{\cnrs}[1][\scad]{\sca[#1]{cnrs}\XS}

	\def\UMR{Unit\'e Mixte de Recherche\XS}
	\newcommand{\umr}[1][\scad]{\sca[#1]{umr}\XS}

	\def\CNES{Centre National d'\'Etudes Spatiales\XS}
	\newcommand{\cnes}[1][\scad]{\sca[#1]{cnes}\XS}

	\def\EDF{\'Electricit\'e de France\XS}
	\newcommand{\edf}[1][\scad]{\sca[#1]{edf}\XS}

	\def\ENSTA{\'Ecole Nationale Sup\'erieure de Techniques Avanc\'ees\XS}
	\newcommand{\ensta}[1][\scad]{\sca[#1]{ensta}\XS}

	\def\ENST{\'Ecole Nationale Sup\'erieure des T\'el\'ecommunications\XS}
	\newcommand{\enst}[1][\scad]{\sca[#1]{enst}\XS}

	\def\ESIEA{\'Ecole Sup\'erieure d'Informatique \'Electronique Automatique\XS}
	\newcommand{\esiea}[1][\scad]{\sca[#1]{esiea}\XS}

	\def\ENSEA{\'Ecole Nationale Sup\'erieure de l'\'Electronique et des ses Applications\XS}
	\newcommand{\ensea}[1][\scad]{\sca[#1]{ensea}\XS}

	\def\GPI{Groupe Probl\`emes Inverses\XS}
	\newcommand{\gpi}[1][\scad]{\sca[#1]{gpi}\XS}

	\def\GSI{Groupe Signal~--~Image\XS}
	\newcommand{\gsi}[1][\scad]{\sca[#1]{gsi}\XS}

	\def\IPB{Institut Polytechnique de Bordeaux\XS}
	\newcommand{\ipb}[1][\scad]{\sca[#1]{ipb}\XS}

	\def\BINP{Bordeaux Institut National Polytechnique\XS}
	\newcommand{\binp}[1][\scad]{\sca[#1]{binp}\XS}

	\def\INSERM{Institut National pour la Sant\'e et la Recherche M\'edicale\XS}
	\newcommand{\inserm}[1][\scad]{\sca[#1]{inserm}\XS}

	\def\CNAM{Conservatoire National des Arts et M\'etiers\XS}
	\newcommand{\cnam}[1][\scad]{\sca[#1]{cnam}\XS}

	\def\OPM{Observatoire de Paris\XS}
	\newcommand{\opm}[1][\scad]{\sca[#1]{opm}\XS}

	\def\INRIA{Institut National de Recherche et Informatique et Automatique\XS}
	\newcommand{\inria}[1][\scad]{\sca[#1]{inria}\XS}

	\def\IAS{Institut d'Astrophysique Spatiale\XS}
	\newcommand{\ias}[1][\scad]{\sca[#1]{ias}\XS}

	\def\IAP{Institut d'Astrophysique de Paris\XS}
	\newcommand{\iap}[1][\scad]{\sca[#1]{iap}\XS}

	\def\IPSN{Institut de Protection et de Suret\'e Nucl\'eaire\XS}
	\newcommand{\ipsn}[1][\scad]{\sca[#1]{ipsn}\XS}

	\def\LSS{Laboratoire des Signaux et Syst\`emes\XS}
	\newcommand{\lss}[1][\scad]{\sca[#1]{lss}\XS}

	\def\LAPS{Laboratoire Automatique, productique, Signal\XS}
	\newcommand{\laps}[1][\scad]{\sca[#1]{laps}\XS}

	\def\LIMS{Laboratoire de l'Int\'egration du Mat\'eriau au Syst\`eme\XS}
	\def\IMS{Int\'egration du Mat\'eriau au Syst\`eme\XS}
	\newcommand{\ims}[1][\scad]{\sca[#1]{ims}\XS}

	\def\IMB{Institut de Math\'ematique de Bordeaux\XS}
	\newcommand{\imb}[1][\scad]{\sca[#1]{imb}\XS}

	\def\LaBRI{Laboratoire Bordelais de Recherche en Informatique\XS}
	\newcommand{\labri}[1][\scad]{\sca[#1]{labri}\XS}

	\def\LIMSI{Laboratoire d'Informatique pour la M\'ecanique et les Sciences de l'Ing\'enieur\XS}
	\newcommand{\limsi}[1][\scad]{\sca[#1]{limsi-cnrs}\XS}

	\def\ONERA{Office National d'\'Etudes et de Recherches A\'erospatiales\XS}
	\newcommand{\onera}[1][\scad]{\sca[#1]{on\'era}\XS}

	\def\CLS{Collecte Localisation Satellites\XS}
	\newcommand{\cls}[1][\scad]{\sca[#1]{cls}\XS}

	\def\SSL{signaux et syst\`emes lin\'eaires\XS}
	\def\GSSL{Signaux et syst\`emes lin\'eaires\XS}
	\newcommand{\ssl}[1][\scad]{\sca[#1]{ssl}\XS}

	\def\IFIPS{Institut de Formation des Ing\'enieurs de Paris-Sud\XS}
	\newcommand{\ifips}[1][\scad]{\sca[#1]{ifips}\XS}

	\def\IST{Information, Syst\`emes et Technologie\XS}
	\newcommand{\isp}[1][\scad]{\sca[#1]{ist}\XS}

	\def\ISC{Ing\'enierie des Syst\`emes Complexes\XS}
	\newcommand{\isc}[1][\scad]{\sca[#1]{isc}\XS}

	\def\pISIS{Ing\'enierie des Syst\`emes pour l'Image et le Signal\XS}
	\newcommand{\pisis}[1][\scad]{\sca[#1]{isis}\XS}

	\def\LMD{Licence, Master, Doctorat\XS}
	\newcommand{\lmd}[1][\scad]{\sca[#1]{lmd}\XS}

   \def\MDC{Ma\^itre de conf\'erences\XS}
   \newcommand{\mdc}[1][\scad]{\sca[#1]{mdc}\XS}

   \def\UPS{Universit\'e Paris-Sud\XS}
   \newcommand{\ups}[1][\scad]{\sca[#1]{ups}\XS}

   \def\UBI{Universit\'e Bordeaux~1\XS}
   \newcommand{\ubI}[1][\scad]{\sca[#1]{ub{\footnotesize 1}}\XS}

   \def\UdB{Universit\'e de Bordeaux\XS}
   \newcommand{\udb}[1][\scad]{\sca[#1]{ub}\XS}

   \def\TdSI{Traitement du Signal et de l'Image\XS}
   \newcommand{\tdsi}[1][\scad]{\sca[#1]{tdsi}\XS}

   \def\SDI{Sciences de l'Ing\'enieur\XS}
   \newcommand{\sdi}[1][\scad]{\sca[#1]{sdi}\XS}



% Unites Thomson
   %\newcommand{\thomair}[1][\scad]{\sca[#1]{Thomson-csf Airsys}\XS}
   %\newcommand{\oscar}[1][\scad]{\sca[#1]{Oscar}\XS}
   %\newcommand{\thomrcm}[1][\scad]{\sca[#1]{Thomson-rcm}\XS}

% Divers à virer...
   % LENA, lena upr640,...
   %\newcommand{\uprlen}[1][\scad]{\sca[#1]{upr}{\footnotesize 640}\XS}
   %\def\LENA{Laboratoire d'Encéphalographie et de Neurophysiologie Appliquée\XS}
   %\newcommand{\lena}[1][\scad]{\sca[#1]{lena}\XS}

   %\newcommand{\UFRPhys}[1][\scad]{{\ufr de physique}\XS}
   %\newcommand{\ups}[1][\scad]{\sca[#1]{ups}\XS}




==> Macros/alphabet.tex <==
% Document LaTeX        Auteur : Guy Le Besnerais       Date : 25/05/94
% Modification : J.-F. Gio      (15/09/95)
%                               J.I. (format Latex 2e, taille adaptative 22/03/99)
%                                    (fonte blackboard 27/08/99)
%
% ==> OK, JFG -- 26/04/2010
%
% Objet : Definitions compactes d'alphabets pour ecriture en Math
% b pour bold italique : \Ab
% v pour bold droit : \Av
% D pour droit : \AD
% c pour cursif : \Ac
% bb pour blackboard : \Abb
% Capitale pour capitale : \Lambda

% \typeout{\space}
% \typeout{\space\space\space\space Fichier 'alphabet.tex' -- LSS 1994/95/99}
% \typeout{\space\space\space\space (necessite les packages xspace, amsmath, bbm)}
% \typeout{\space}

\RequirePackage{amsmath}
\RequirePackage{xspace}
%\RequirePackage{bbm}
\RequirePackage{dsfont}
\RequirePackage{oldgerm}		% 04.06.2003   Pour les alphabet Gothiques

%-------------------------------------------

% DEFINITIONS PRELIMINAIRES 

\def\XS{\xspace}
\DeclareMathAlphabet{\mathb}{OML}{cmm}{b}{it}
\def\sbm#1{\ensuremath{\mathb{#1}}}                % Style gras italique (necessite amsmath)           
%
\def\sbmm#1{\ensuremath{\boldsymbol{#1}}}          % Style gras italique (necessite amsmath)           
\def\sdm#1{\ensuremath{\mathrm{#1}}}               % Style droit en math
\def\sbv#1{\ensuremath{\mathbf{#1}}}               % Style gras droit
\def\scu#1{\ensuremath{\mathcal{#1\XS}}}           % Style cursif
\def\scb#1{\ensuremath{\boldsymbol{\mathcal{#1}}}} % Style gras cursif

%\def\sbl#1{\ensuremath{\mathbbm{#1}}}              % Style blackboard (necessite bbm)
\def\sbl#1{\ensuremath{\mathds{#1}}}              % Style blackboard (necessite bbm)

%-------------------------------------------

% ALPHABET GRAS ITALIQUE, taille adaptative

\def\Ab{{\sbm{A}}\XS}  \def\ab{{\sbm{a}}\XS}
\def\Bb{{\sbm{B}}\XS}  \def\bb{{\sbm{b}}\XS}
\def\Cb{{\sbm{C}}\XS}  \def\cb{{\sbm{c}}\XS}
\def\Db{{\sbm{D}}\XS}  \def\db{{\sbm{d}}\XS}
\def\Eb{{\sbm{E}}\XS}  \def\eb{{\sbm{e}}\XS}
\def\Fb{{\sbm{F}}\XS}  \def\fb{{\sbm{f}}\XS}
\def\Gb{{\sbm{G}}\XS}  \def\gb{{\sbm{g}}\XS}
\def\Hb{{\sbm{H}}\XS}  \def\hb{{\sbm{h}}\XS}
\def\Ib{{\sbm{I}}\XS}  \def\ib{{\sbm{i}}\XS}
\def\Jb{{\sbm{J}}\XS}  \def\jb{{\sbm{j}}\XS}
\def\Kb{{\sbm{K}}\XS}  \def\kb{{\sbm{k}}\XS}
\def\Lb{{\sbm{L}}\XS}  \def\lb{{\sbm{l}}\XS}
\def\Mb{{\sbm{M}}\XS}  \def\mb{{\sbm{m}}\XS}
\def\Nb{{\sbm{N}}\XS}  \def\nb{{\sbm{n}}\XS}
\def\Ob{{\sbm{O}}\XS}  \def\ob{{\sbm{o}}\XS}
\def\Pb{{\sbm{P}}\XS}  \def\pb{{\sbm{p}}\XS}
\def\Qb{{\sbm{Q}}\XS}  \def\qb{{\sbm{q}}\XS}
\def\Rb{{\sbm{R}}\XS}  \def\rb{{\sbm{r}}\XS}
\def\Sb{{\sbm{S}}\XS}  \def\sb{{\sbm{s}}\XS}
\def\Tb{{\sbm{T}}\XS}  \def\tb{{\sbm{t}}\XS}
\def\Ub{{\sbm{U}}\XS}  \def\ub{{\sbm{u}}\XS}
\def\Vb{{\sbm{V}}\XS}  \def\vb{{\sbm{v}}\XS}
\def\Wb{{\sbm{W}}\XS}  \def\wb{{\sbm{w}}\XS}
\def\Xb{{\sbm{X}}\XS}  \def\xb{{\sbm{x}}\XS}
\def\Yb{{\sbm{Y}}\XS}  \def\yb{{\sbm{y}}\XS}
\def\Zb{{\sbm{Z}}\XS}  \def\zb{{\sbm{z}}\XS}


% ALPHABET CURSIF MAJUSCULE, taille adaptative
% Cursif,               % Cursif gras

\def\Ac{{\scu{A}}\XS}   \def\Acb{{\scb{A}}\XS}
\def\Bc{{\scu{B}}\XS}   \def\Bcb{{\scb{B}}\XS}
\def\Cc{{\scu{C}}\XS}   \def\Ccb{{\scb{C}}\XS}
\def\Dc{{\scu{D}}\XS}   \def\Dcb{{\scb{D}}\XS}
\def\Ec{{\scu{E}}\XS}   \def\Ecb{{\scb{E}}\XS}
\def\Fc{{\scu{F}}\XS}   \def\Fcb{{\scb{F}}\XS}
\def\Gc{{\scu{G}}\XS}   \def\Gcb{{\scb{G}}\XS}
\def\Hc{{\scu{H}}\XS}   \def\Hcb{{\scb{H}}\XS}
\def\Ic{{\scu{I}}\XS}   \def\Icb{{\scb{I}}\XS}
\def\Jc{{\scu{J}}\XS}   \def\Jcb{{\scb{J}}\XS}
\def\Kc{{\scu{K}}\XS}   \def\Kcb{{\scb{K}}\XS}
\def\Lc{{\scu{L}}\XS}   \def\Lcb{{\scb{L}}\XS}
\def\Mc{{\scu{M}}\XS}   \def\Mcb{{\scb{M}}\XS}
\def\Nc{{\scu{N}}\XS}   \def\Ncb{{\scb{N}}\XS}
\def\Oc{{\scu{O}}\XS}   \def\Ocb{{\scb{O}}\XS}
\def\Pc{{\scu{P}}\XS}   \def\Pcb{{\scb{P}}\XS}
\def\Qc{{\scu{Q}}\XS}   \def\Qcb{{\scb{Q}}\XS}
\def\Rc{{\scu{R}}\XS}   \def\Rcb{{\scb{R}}\XS}
\def\Sc{{\scu{S}}\XS}   \def\Scb{{\scb{S}}\XS}
\def\Tc{{\scu{T}}\XS}   \def\Tcb{{\scb{T}}\XS}
\def\Uc{{\scu{U}}\XS}   \def\Ucb{{\scb{U}}\XS}
\def\Vc{{\scu{V}}\XS}   \def\Vcb{{\scb{V}}\XS}
\def\Wc{{\scu{W}}\XS}   \def\Wcb{{\scb{W}}\XS}
\def\Xc{{\scu{X}}\XS}   \def\Xcb{{\scb{X}}\XS}
\def\Yc{{\scu{Y}}\XS}   \def\Ycb{{\scb{Y}}\XS}
\def\Zc{{\scu{Z}}\XS}   \def\Zcb{{\scb{Z}}\XS}


% ALPHABET DROIT EN MATHS, taille adaptative

\def\AD{{\sdm{A}}\XS}  \def\aD{{\sdm{a}}\XS}
\def\BD{{\sdm{B}}\XS}  \def\bD{{\sdm{b}}\XS}
\def\CD{{\sdm{C}}\XS}  \def\cD{{\sdm{c}}\XS}
\def\DD{{\sdm{D}}\XS}  \def\dD{{\sdm{d}}\XS}
\def\ED{{\sdm{E}}\XS}  \def\eD{{\sdm{e}}\XS}
\def\FD{{\sdm{F}}\XS}  \def\fD{{\sdm{f}}\XS}
\def\GD{{\sdm{G}}\XS}  \def\gD{{\sdm{g}}\XS}
\def\HD{{\sdm{H}}\XS}  \def\hD{{\sdm{h}}\XS}
\def\ID{{\sdm{I}}\XS}  \def\iD{{\sdm{i}}\XS}
\def\JD{{\sdm{J}}\XS}  \def\jD{{\sdm{j}}\XS}
\def\KD{{\sdm{K}}\XS}  \def\kD{{\sdm{k}}\XS}
\def\LD{{\sdm{L}}\XS}  \def\lD{{\sdm{l}}\XS}
\def\MD{{\sdm{M}}\XS}  \def\mD{{\sdm{m}}\XS}
\def\ND{{\sdm{N}}\XS}  \def\nD{{\sdm{n}}\XS}
\def\OD{{\sdm{O}}\XS}  \def\oD{{\sdm{o}}\XS}
\def\PD{{\sdm{P}}\XS}  \def\pD{{\sdm{p}}\XS}
\def\QD{{\sdm{Q}}\XS}  \def\qD{{\sdm{q}}\XS}
\def\RD{{\sdm{R}}\XS}  \def\rD{{\sdm{r}}\XS}
\def\SD{{\sdm{S}}\XS}  \def\sD{{\sdm{s}}\XS}
\def\TD{{\sdm{T}}\XS}  \def\tD{{\sdm{t}}\XS}
\def\UD{{\sdm{U}}\XS}  \def\uD{{\sdm{u}}\XS}
\def\VD{{\sdm{V}}\XS}  \def\vD{{\sdm{v}}\XS}
\def\WD{{\sdm{W}}\XS}  \def\wD{{\sdm{w}}\XS}
\def\XD{{\sdm{X}}\XS}  \def\xD{{\sdm{x}}\XS}
\def\YD{{\sdm{Y}}\XS}  \def\yD{{\sdm{y}}\XS}
\def\ZD{{\sdm{Z}}\XS}  \def\zD{{\sdm{z}}\XS}


% ALPHABET GRAS DROIT, taille adaptative

\def\Av{{\sbv{A}}\XS}  \def\av{{\sbv{a}}\XS}
\def\Bv{{\sbv{B}}\XS}  \def\bv{{\sbv{b}}\XS}
\def\Cv{{\sbv{C}}\XS}  \def\cv{{\sbv{c}}\XS}
\def\Dv{{\sbv{D}}\XS}  \def\dv{{\sbv{d}}\XS}
\def\Ev{{\sbv{E}}\XS}  \def\ev{{\sbv{e}}\XS}
\def\Fv{{\sbv{F}}\XS}  \def\fv{{\sbv{f}}\XS}
\def\Gv{{\sbv{G}}\XS}  \def\gv{{\sbv{g}}\XS}
\def\Hv{{\sbv{H}}\XS}  \def\hv{{\sbv{h}}\XS}
\def\Iv{{\sbv{I}}\XS}  \def\iv{{\sbv{i}}\XS}
\def\Jv{{\sbv{J}}\XS}  \def\jv{{\sbv{j}}\XS}
\def\Kv{{\sbv{K}}\XS}  \def\kv{{\sbv{k}}\XS}
\def\Lv{{\sbv{L}}\XS}  \def\lv{{\sbv{l}}\XS}
\def\Mv{{\sbv{M}}\XS}  \def\mv{{\sbv{m}}\XS}
\def\Nv{{\sbv{N}}\XS}  \def\nv{{\sbv{n}}\XS}
\def\Ov{{\sbv{O}}\XS}  \def\ov{{\sbv{o}}\XS}
\def\Pv{{\sbv{P}}\XS}  \def\pv{{\sbv{p}}\XS}
\def\Qv{{\sbv{Q}}\XS}  \def\qv{{\sbv{q}}\XS}
\def\Rv{{\sbv{R}}\XS}  \def\rv{{\sbv{r}}\XS}
\def\Sv{{\sbv{S}}\XS}  \def\sv{{\sbv{s}}\XS}
\def\Tv{{\sbv{T}}\XS}  \def\tv{{\sbv{t}}\XS}
\def\Uv{{\sbv{U}}\XS}  \def\uv{{\sbv{u}}\XS}
\def\Vv{{\sbv{V}}\XS}  \def\vv{{\sbv{v}}\XS}
\def\Wv{{\sbv{W}}\XS}  \def\wv{{\sbv{w}}\XS}
\def\Xv{{\sbv{X}}\XS}  \def\xv{{\sbv{x}}\XS}
\def\Yv{{\sbv{Y}}\XS}  \def\yv{{\sbv{y}}\XS}
\def\Zv{{\sbv{Z}}\XS}  \def\zv{{\sbv{z}}\XS}


% Nouveau (08/99) : ALPHABET BLACKBOARD, taille adaptative

\def\Abb{{\sbl{A}}\XS}  \def\abb{{\sbl{a}}\XS}
\def\Bbb{{\sbl{B}}\XS}  \def\bbb{{\sbl{b}}\XS}
\def\Cbb{{\sbl{C}}\XS}  \def\cbb{{\sbl{c}}\XS}
\def\Dbb{{\sbl{D}}\XS}  \def\dbb{{\sbl{d}}\XS}
\def\Ebb{{\sbl{E}}\XS}  \def\ebb{{\sbl{e}}\XS}
\def\Fbb{{\sbl{F}}\XS}  \def\fbb{{\sbl{f}}\XS}
\def\Gbb{{\sbl{G}}\XS}  \def\gbb{{\sbl{g}}\XS}
\def\Hbb{{\sbl{H}}\XS}  \def\hbb{{\sbl{h}}\XS}
\def\Ibb{{\sbl{I}}\XS}  \def\ibb{{\sbl{i}}\XS}
\def\Jbb{{\sbl{J}}\XS}  \def\jbb{{\sbl{j}}\XS}
\def\Kbb{{\sbl{K}}\XS}  \def\kbb{{\sbl{k}}\XS}
\def\Lbb{{\sbl{L}}\XS}  \def\lbb{{\sbl{l}}\XS}
\def\Mbb{{\sbl{M}}\XS}  \def\mbb{{\sbl{m}}\XS}
\def\Nbb{{\sbl{N}}\XS}  \def\nbb{{\sbl{n}}\XS}
\def\Obb{{\sbl{O}}\XS}  \def\obb{{\sbl{o}}\XS}
\def\Pbb{{\sbl{P}}\XS}  \def\pbb{{\sbl{p}}\XS}
\def\Qbb{{\sbl{Q}}\XS}  \def\qbb{{\sbl{q}}\XS}
\def\Rbb{{\sbl{R}}\XS}  \def\rbb{{\sbl{r}}\XS}
\def\Sbb{{\sbl{S}}\XS}  \def\sbb{{\sbl{s}}\XS}
\def\Tbb{{\sbl{T}}\XS}  \def\tbb{{\sbl{t}}\XS}
\def\Ubb{{\sbl{U}}\XS}  \def\ubb{{\sbl{u}}\XS}
\def\Vbb{{\sbl{V}}\XS}  \def\vbb{{\sbl{v}}\XS}
\def\Wbb{{\sbl{W}}\XS}  \def\wbb{{\sbl{w}}\XS}
\def\Xbb{{\sbl{X}}\XS}  \def\xbb{{\sbl{x}}\XS}
\def\Ybb{{\sbl{Y}}\XS}  \def\ybb{{\sbl{y}}\XS}
\def\Zbb{{\sbl{Z}}\XS}  \def\zbb{{\sbl{z}}\XS}

% ALPHABET GREC GRAS italique, taille adaptative

\def\alphab      {{\sbmm{\alpha}}\XS}
\def\betab       {{\sbmm{\beta}}\XS}
\def\gammab      {{\sbmm{\gamma}}\XS}      \def\Gammab    {{\sbmm{\Gamma}}\XS}
\def\deltab      {{\sbmm{\delta}}\XS}      \def\Deltab    {{\sbmm{\Delta}}\XS}
\def\epsilonb    {{\sbmm{\epsilon}}\XS}
\def\varepsilonb {{\sbmm{\varepsilon}}\XS}
\def\etab        {{\sbmm{\eta}}\XS}
\def\thetab      {{\sbmm{\theta}}\XS}      \def\Thetab    {{\sbmm{\Theta}}\XS}
\def\varthetab   {{\sbmm{\vartheta}}\XS}
\def\iotab       {{\sbmm{\iota}}\XS}
\def\kappab      {{\sbmm{\kappa}}\XS}
\def\varkappab   {{\sbmm{\varkappa}}\XS}
\def\lambdab     {{\sbmm{\lambda}}\XS}     \def\Lambdab   {{\sbmm{\Lambda}}\XS}
\def\mub         {{\sbmm{\mu}}\XS}
\def\nub         {{\sbmm{\nu}}\XS}
\def\xib         {{\sbmm{\xi}}\XS}         \def\Xib       {{\sbmm{\Xi}}\XS}
\def\pib         {{\sbmm{\pi}}\XS}         \def\Pib       {{\sbmm{\Pi}}\XS}
\def\varpib      {{\sbmm{\varpi}}\XS}
\def\rhob        {{\sbmm{\rho}}\XS}
\def\varrhob     {{\sbmm{\varrho}}\XS}
\def\sigmab      {{\sbmm{\sigma}}\XS}      \def\Sigmab    {{\sbmm{\Sigma}}\XS}
\def\varsigmab   {{\sbmm{\varsigma}}\XS}   \def\Varsigmab {{\sbmm{\Varsigma}}\XS}
\def\phib        {{\sbmm{\phi}}\XS}        \def\Phib      {{\sbmm{\Phi}}\XS}
\def\varphib     {{\sbmm{\varphi}}\XS}
\def\chib        {{\sbmm{\chi}}\XS}
\def\psib        {{\sbmm{\psi}}\XS}        \def\Psib      {{\sbmm{\Psi}}\XS}
\def\omegab      {{\sbmm{\omega}}\XS}      \def\Omegab    {{\sbmm{\Omega}}\XS}
\def\taub        {{\sbmm{\tau}}\XS}
\def\upsilonb    {{\sbmm{\upsilon}}\XS}   \def\Upsilonb  {{\sbmm{\Upsilon}}\XS}
\def\zetab       {{\sbmm{\zeta}}\XS}

\def\ellb{{\sbmm{\ell}}\XS}


% CHIFFRES
% Gras et Blackboard, taille adaptative

\def\zerob   {{\sbv{0}}\XS}        \def\zerobb   {{\sbl{O}}\XS}
\def\unb     {{\sbv{1}}\XS}        \def\unbb     {{\sbl{1}}\XS}
\def\deuxb   {{\sbv{2}}\XS}        \def\deuxbb   {{\sbl{2}}\XS}
\def\troisb  {{\sbv{3}}\XS}        \def\troisbb  {{\sbl{3}}\XS}
\def\quatreb {{\sbv{4}}\XS}        \def\quatrebb {{\sbl{4}}\XS}
\def\cinqb   {{\sbv{5}}\XS}        \def\cinqbb   {{\sbl{5}}\XS}
\def\sixb    {{\sbv{6}}\XS}        \def\sixbb    {{\sbl{6}}\XS}
\def\septb   {{\sbv{7}}\XS}        \def\septbb   {{\sbl{7}}\XS}
\def\huitb   {{\sbv{8}}\XS}        \def\huitbb   {{\sbl{8}}\XS}
\def\neufb   {{\sbv{9}}\XS}        \def\neufbb   {{\sbl{9}}\XS}


% QUELQUES ENSEMBLES

\def\eC{\Cbb}
\def\eE{\Ebb}
\def\eN{\Nbb}
\def\eQ{\Qbb}
\def\eR{\Rbb}
\def\eZ{\Zbb}
\def\eK{\Kbb}

% ALPHABET GOTHIQUES  04.06.2003  M.M. ICHIR

\def\Ag{{\textgoth{A}}\XS}  \def\ag{{\textgoth{a}}\XS}
\def\Bg{{\textgoth{B}}\XS}  \def\bg{{\textgoth{b}}\XS}
\def\Cg{{\textgoth{C}}\XS}  \def\cg{{\textgoth{c}}\XS}
\def\Dg{{\textgoth{D}}\XS}  \def\dg{{\textgoth{d}}\XS}
\def\Eg{{\textgoth{E}}\XS}  \def\eg{{\textgoth{e}}\XS}
\def\Fg{{\textgoth{F}}\XS}  \def\fg{{\textgoth{f}}\XS}
\def\Gg{{\textgoth{G}}\XS}  %\def\gg{{\textgoth{g}}\XS}
\def\Hg{{\textgoth{H}}\XS}  \def\hg{{\textgoth{h}}\XS}
\def\Ig{{\textgoth{I}}\XS}  \def\ig{{\textgoth{i}}\XS}
\def\Jg{{\textgoth{J}}\XS}  \def\jg{{\textgoth{j}}\XS}
\def\Kg{{\textgoth{K}}\XS}  \def\kg{{\textgoth{k}}\XS}
\def\Lg{{\textgoth{L}}\XS}  \def\lg{{\textgoth{l}}\XS}
\def\Mg{{\textgoth{M}}\XS}  \def\mg{{\textgoth{m}}\XS}
\def\Ng{{\textgoth{N}}\XS}  \def\ng{{\textgoth{n}}\XS}
\def\Og{{\textgoth{O}}\XS}  \def\og{{\textgoth{o}}\XS}
\def\Pg{{\textgoth{P}}\XS}  \def\pg{{\textgoth{p}}\XS}
\def\Qg{{\textgoth{Q}}\XS}  \def\qg{{\textgoth{q}}\XS}
\def\Rg{{\textgoth{R}}\XS}  \def\rg{{\textgoth{r}}\XS}
\def\Sg{{\textgoth{S}}\XS}  \def\sg{{\textgoth{s}}\XS}
\def\Tg{{\textgoth{T}}\XS}  \def\tg{{\textgoth{t}}\XS}
\def\Ug{{\textgoth{U}}\XS}  \def\ug{{\textgoth{u}}\XS}
\def\Vg{{\textgoth{V}}\XS}  \def\vg{{\textgoth{v}}\XS}
\def\Wg{{\textgoth{W}}\XS}  \def\wg{{\textgoth{w}}\XS}
\def\Xg{{\textgoth{X}}\XS}  \def\xg{{\textgoth{x}}\XS}
\def\Yg{{\textgoth{Y}}\XS}  \def\yg{{\textgoth{y}}\XS}
\def\Zg{{\textgoth{Z}}\XS}  \def\zg{{\textgoth{z}}\XS}

